On Out-of-Distribution Detection for Audio with Deep Nearest Neighbors

Out-of-distribution (OOD) detection is concerned with identifying data points that do not belong to the same distribution as the model's training data. For the safe deployment of predictive models in a real-world environment, it is critical to avoid making confident predictions on OOD inputs as it can lead to potentially dangerous consequences. However, OOD detection largely remains an under-explored area in the audio (and speech) domain. This is despite the fact that audio is a central modality for many tasks, such as speaker diarization, automatic speech recognition, and sound event detection. To address this, we propose to leverage feature-space of the model with deep k-nearest neighbors to detect OOD samples. We show that this simple and flexible method effectively detects OOD inputs across a broad category of audio (and speech) datasets. Specifically, it improves the false positive rate (FPR@TPR95) by 17% and the AUROC score by 7% than other prior techniques.

==> rebuttal.tex <==
We are grateful for the time and effort taken by the reviewers in providing their valuable insights. In light of the received feedback, we will make revision to the paper to emphasize the above-mentioned points. We also want to mention that we will make code available to facilitate further research in this area.

Response to Reviewer #1

Thank you for the feedback and valuable comments. We want to emphasize that our work represents the first attempt in the examination of out-of-distribution (OOD) phenomena for deep models in the audio domain, as acknowledged in the review. The simplicity of the method is one of its strengths as it allows for easy implementation and interpretation of the results (see further details below). Through an extensive evaluation of various existing techniques for OOD detection across a diverse array of classification benchmark datasets, we have established the superior performance of our k-nearest neighbor-based method, which also boasts a highly simplistic implementation, as we highlighted throughout the paper.

There are several challenges for robust OOD detection for deep audio classifiers, including variety (and similarity originating from same recording equipment and environmental settings) of audio recording, similar sounding keywords and noise patterns can also contribute to the difficulty in accurately identifying OOD samples, as they may result in sounds that are similar despite having different class labels. Given these challenges, we believe the k-nearest neighbor (kNN) approach is the most robust technique as shown by extensive experimentation. This is due to the utilization of distances in the learned embedding space, wherein the kNN algorithm compares the distance of a given sample to the k closest training set embeddings and flags it as OOD if the distance exceeds a certain threshold. Other methods, such as ODIN and GradNorm, lack this explicit perspective as kNN does by having access to entire training set embedding, while ODIN and GradNorm rely solely on the gradient information of the sample in question to determine its OOD status.  As our results indicate, utilizing the embedding space provides a more informative signal for identifying OOD samples than simply relying on softmax scores or gradient information alone.

Further, our proposed approach offers a transparent and interpretable method for identifying OOD samples within the context of audio classification. Specifically, by detecting the k closest samples in the embedding space and their corresponding distances, a human operator can verify the OOD identification through listening to the k closest training set audio examples and the test example. This not only facilitates model improvement through refinement of the data collection pipeline, but also strengthens the confidence in the OOD detection method and can be used to provide explanations. 

Response to Reviewer #2

Thank you very much for your encouraging feedback. We believe the utilized benchmarking datasets are well-known and greatly covers the complexity of the OOD detection problem ranging from keyword spotting, environmental sounds, language identification among others. Nevertheless, further validation of the proposed method's robustness would be fruitful through its deployment in real-world scenarios, which is outside the scope of current work. 

As our paper is the first attempt at studying OOD in audio-domain we focused on multi-class classification setting. In future, we aim to study how our method would work in a multi-label classification setting, such as for models trained on AudioSet dataset. We note that it would require to have other test datasets labeled for multi-label classification problems. 

Response to Reviewer #3

Thank you very much for the encouraging feedback. 


